Training for the Future: A Simple Gradient Interpolation Loss to Generalize Along Time

In several real world applications, machine learning models are deployed to make predictions on data whose distribution changes gradually along time, leading to a drift between the train and test distributions. Such models are often re-trained on new data periodically, and they hence need to generalize to data not too far into the future. In this context, there is much prior work on enhancing temporal generalization, e.g. continuous transportation of past data, kernel smoothed time-sensitive parameters and more recently, adversarial learning of time-invariant features. However, these methods share several limitations, e.g, poor scalability, training instability, and dependence on unlabeled data from the future. Responding to the above limitations, we propose a simple method that starts with a model with time-sensitive parameters but regularizes its temporal complexity using a Gradient Interpolation (GI) loss. GI allows the decision boundary to change along time and can still prevent overfitting to the limited training time snapshots by allowing task-specific control over changes along time. We compare our method to existing baselines on multiple real-world datasets, which show that GI outperforms more complicated generative and adversarial approaches on the one hand, and simpler gradient regularization methods on the other.

==> NeurIPS/sections/checklist.tex <==
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{We refer the reader to sec~\ref{sec:Conclusion} for a list of limitations of our work} 
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{We discuss this in the supplemental material}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We include the code in the supplemental material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We report this information in the supplemental material}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We report all results over 5 random restarts}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We report this information in the supplemental material}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We list this information in the References}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> NeurIPS/sections/expt_tables.tex <==
% Contains raw/unformatted tables from experiments.tex
% Mainly for our reference and to clean up the source tex 

% \begin{table}[!htp]
%   \caption{Accuracy for various classifcation algorithms on the datasets discussed above}
  
%   \centering
%   \begin{tabular}{p{3cm}p{2.0cm}p{2.0cm}p{2.0cm}}
%     \toprule
%     Algorithm & 2-Moons & Rot-MNIST & Sleep \\
%     \midrule
%     \baseline & 0.87 (0.05) & 81.4 (4.0) & 65.8 (0.61) \\
%     \our & 0.922 (0.03) & 90.9 (1.1) & 69.61 (1.1)\\
%     \goodfellow~\cite{GoodfellowPerturbs14} & 0.915 (0.04) & 89.5 (0.9) &  \\
%     \cida~\cite{wang2020continuously} & & 92.2 (1.5) & &\\
%     % \textcolor{red}{CDOT} &  &  & \\
%     \incFinetune &  & 83.1 (4.0) &   & \\
    
%     \bottomrule
%   \end{tabular}
%   \label{tab:main_classification}
% \end{table}


\iffalse
    
    \begin{table}[!htp]
      \caption{Accuracy for various classification algorithms on the datasets described in section \ref{sec:expt:data}. The standard deviation is reported in parentheses.}
      \centering
      \begin{tabular}{|p{3cm}|c|c|c|}
        \hline \rule{0pt}{12pt}
        \textbf{Algorithm} & \textbf{2-Moons} & \textbf{Rot-MNIST} & Sleep \\
        \hline
        \baseline & 77.6 (3.6) & 81.4 (4.0) & {65.8 (0.6)} \\
        % \tbaseline & & 82.7 (3.7) & 94.52 (3.5) & 68.82 (0.96)\\
        % \baseTRelu & & 82.1 (4.3) &  & 68.61 (1.03)\\
        \our & 96.5 (1.4)  & 92.3 (1.3) & 69.6 (1.1)\\
        % GI with KL & 95.1 (2.1)  & 91.2 (1.4) & & \\
        \goodfellow~\cite{GoodfellowPerturbs14} & 90.4 (2.4) & 90.5 (1.4) &  \\
        \cida & 89.15 (1.7) & 90.7 (0.7) & \\
        % CDOT &  &  & \\
    % \adagraph \\
        \incFinetune & 89.25 (1.8) & 90.9 (0.8) &\\
        %\tincFinetune & 91.0 (1.8) & 91.4 (1.1)&  69.47 (1.00) \\
        \ordinalclassifier & & 88.0 (0.8) & \\
        %\ode & & & \\
    
        \bottomrule
      \end{tabular}
      \label{tab:main_classification}
    \end{table}
    
    
    % MNIST & Rot-MNIST (full)
    % ) & 92.98 (3.7)
    % ) & 96.04 (4.0)
    % &  93.72 (3.7) 
    %  & 95.56 (4.1) 
    
    % \begin{table}[!htp]
    %   \caption{MSE for various regression algorithms on the datasets discussed above}
      
    %   \centering
    %   \begin{tabular}{p{3cm}p{2.5cm}p{2.5cm}}
    %     \toprule
    %     Algorithm & House Prices & M5 & \\
    %     \midrule
    %     \baseline & 10.532 (0.62) & 0.4593 (0.49)  \\
    %     \baseTRelu & & 0.2773 (0.18) \\
    %     \our & 10.178 (0.15) & 0.1554 (0.15) \\
    %     \cida & 10.316 (0.51) &  \\
    %     \goodfellow & 9.978 (0.07) &   \\
    %     Inc-finetune &  &   0.3884 (0.34) \\
    %     T-Inc-finetune &  & \\
    %     \bottomrule
    %   \end{tabular}
    %   \label{tab:mnist}
    % \end{table}
    
    % \begin{table}[!h]
    %   \caption{MSE for various regression algorithms on the datasets discussed above}
      
    %   \centering
    %   \begin{tabular}{p{3cm}p{2.5cm}p{2.5cm}p{2.5cm}}
    %     \toprule
    %     Algorithm & House Prices & M5 Hobbies & M5 Household\\
    %     \midrule
    %     \baseline & 10.97 (0.36) & 0.4593  (0.49)  & 0.3327 (0.1)\\
        
    %     \our & 9.64 (0.02) & 0.1554 (0.15) & 0.1107 (0.07)\\
    %     \cida $^{*}$ & 9.69 (0.06) &  &\\
    %     \goodfellow & 9.74 (0.04) &  0.1774 (0.17) & 0.1104 (0.06)\\
    %     \incFinetune &  9.70 (0.01) &   0.3884 (0.34) \\
      
    %     \bottomrule
    %   \end{tabular}
    %   \label{tab:mnist}
    % \end{table}
\fi



\iffalse
    \baseline & 10.97 (0.36) & 0.4593  (0.49)  & 0.3327 (0.1)\\
    % \tbaseline & 11.00 (0.15) & 0.3768  (0.21) &\\
    % \baseTRelu & 11.25 (0.30) & 0.2773  (0.18) & 0.1397 (0.08)\\
    \our & 9.64 (0.02) & 0.1554 (0.15) & 0.1107 (0.07)\\
    \cida $^{*}$ & 9.69 (0.06) &  &\\
    \goodfellow & 9.74 (0.04) &  0.1774 (0.17) & 0.1104 (0.06)\\
    \incFinetune &  9.70 (0.01) &   0.3884 (0.34) &\\
\fi
\iffalse
    
    \begin{table}[!h]
      \caption{Performance for various regression algorithms on the datasets described in section \ref{sec:expt:data}. The standard deviation is reported in parentheses.}
      
      \centering
      \begin{tabular}{|p{3cm}|l|l|l|}
        \hline
        \rule{0pt}{12pt}
        Algorithm & House Prices (MAE) & M5 Hobbies (MSE) & M5 Household (MSE)\\
        \hline
        \baseline & 10.97 (0.36) & 0.46  (0.49)  & 0.33 (0.10)\\
        % \tbaseline & 11.00 (0.15) & 0.3768  (0.21) &\\
        % \baseTRelu & 11.25 (0.30) & 0.2773  (0.18) & 0.1397 (0.08)\\
        \our & 9.64 (0.02) & 0.16 (0.15) & 0.11 (0.07)\\
        \cida $^{*}$ & 9.69 (0.06) & 0.27 (0.42) &\\
        \goodfellow & 9.74 (0.04) &  0.18 (0.17) & 0.11 (0.06)\\
        \incFinetune &  9.70 (0.01) &   0.39 (0.34) &\\
        % \tincFinetune & 9.83 (0.08) & &\\
        % IncFinetune-TReLU & & 0.1568 (0.15) & 0.1108 (0.07) \\
        \ordinalclassifier & & & \\
        \ode & & & \\
    
        \bottomrule
      \end{tabular}
      \label{tab:main_regression}
    \end{table}
\fi

%\begin{table}[!htp]
%  \caption{Accuracy for various algorithm}
  
%  \centering
%  \begin{tabular}{p{3cm}p{2cm}p{2cm}}
%    \toprule
%    Algorithm & Accuracy $(60^{\circ})$ & Accuracy $(75^{\circ})$ \\
%    \midrule
%    Source Only & 88.4 (1.7) &  \\
%    GI & 89.5 (1.5) & 80.4 \\
%    Goodfellow & 89.5 (1.6) & 80.4 \\
%    CIDA & 90.9 & \\
%    CDOT & 85.0 &  \\
%    Inc-finetune & 85.2 & 72.7 \\
%    T-Inc-finetune & 88.0 & 74.2 \\
%    \bottomrule
%  \end{tabular}
%  \label{tab:mnist}
%\end{table}

%\begin{table}[!htp]
%  \caption{Rotated 2-moons accuracy for various algorithm}
  
%  \centering
%  \begin{tabular}{p{3cm}p{2cm}p{2cm}}
%    \toprule
%    Algorithm & Accuracy $(162^{\circ})$ & Accuracy $(180^{\circ})$ \\
%    \midrule
%    Source Only & 0.87 (0.05) &  \\
%    GI & 0.922 (0.03) &  \\
%    Goodfellow &0.915 (0.04) & \\
%    CIDA & 85.5 & \\
%    CDOT & 79.0 &  \\
%    Inc-finetune & 68.5 & \\
%    T-Inc-finetune & 96.5& \\
%    \bottomrule
%  \end{tabular}
%  \label{tab:moons}
%\end{table}

%\begin{table}[!htp]
%  \caption{House Prices error for various algorithm}
  
%  \centering
%  \begin{tabular}{p{3cm}p{2cm}p{2cm}}
%    \toprule
%    Algorithm & Mean Squared Error &  \\
%    \midrule
%    Source Only & 10.532 (0.62)&  \\
%    GI & 10.178 (0.15) &  \\
%    CIDA & 10.316 (0.51) & \\
%    Goodfellow & 9.978 (0.07) &
%    Inc-finetune & 10.412 & \\
%    T-Inc-finetune & 10.018 & \\
%    \bottomrule
%  \end{tabular}
%  \label{tab:moons}
%\end{table}




% \begin{table}[!h]
%   \caption{}
  
%   \centering
%   \begin{tabular}{p{3cm}p{2.0cm}p{2.0cm}p{2.0cm}}
%     \toprule
%     Algorithm & House Prices & M5 (hobbies) & M5 (foods)   \\
%     \midrule
%     \our - e.g & & 0.1568 & \\
%     \our - batch &   & 0.1554 & \\
%     \our - epoch &   & 0.1816 & \\
%     \bottomrule
%   \end{tabular}
%   \label{tab:mnist}
% \end{table}


\begin{table}[!htp]

\caption{Different ways of fine-tuning - Regression tasks}
\centering
\begin{tabular}{llll}
\toprule
\textbf{Ablation}  & \textbf{Housing}    & \textbf{M5 household} & \textbf{M5 hobbies}\\
\midrule
\tbaseline &  & 0.2773 (0.18) & 0.1397 (0.08)\\
\tgoodfellow    &               &               \\
\gradreg       &             &               \\
\curvereg      &              & -- (Didn't converge)    \\
\our & & & \\

\bottomrule
\end{tabular}
\label{tab:ablation_finetune_1}
\end{table}


\begin{table}[!htp]
\centering
\begin{tabular}{|p{3cm}|c|c|c|c|c|}
\hline \rule{0pt}{12pt}
\textbf{Ablation}  & \textbf{\moons}    & \textbf{\rmnist} & \textbf{\house} & \textbf{\hobbies} & \textbf{\household}\\
\hline
\baseline  & & & & & \\
\tbaseline & 95.9\,/\,0.87 & 10.3\,/\,0.9 & & 0.17 \,/\,0.09 & \\
\tincFinetune & 91.25\,/\,8.7 & & & 0.03\,/\,0.02 &\\
\gradreg & \textcolor{red}{77.4 (8.10)} & 11.5\,/\,1.5 & & - & \\
%\curvereg      &    81.4\,/\,16.8      & - & & - &   \\
\tgoodfellow    & 96.7\,/\,0.40 & 9.9\,/\,0.7    &    & &  \\
\our & 96.5\,/\,1.37 & 7.7\,/\,1.3 &  & 0.02\,/\,0.01 & \\
 %GI 3 step & 9.68(0.2) & 91.5 (1.3) \\
 %Multistep & 9.71 (0.02) & 91.1 (1.4) \\
\bottomrule
\end{tabular}
\label{tab:ablation_finetune}
\caption{Disentangling reasons for GI's gains}
\end{table}


==> NeurIPS/sections/intro_old.tex <==
% The paradigm of Machine Learning model training is to collect labeled data, train the model and deploy. The temporal shift between the train and deployment setting is evident; The train data is outdatad, albeit to varying extent depending on the task, for any future use. The problem due to temporal shift has varying effect for different applications. For example, a bird or animal classifier engine trained from data from a decade ago could work just as well now since species evolution is a slow process, although we assume that the picture quality was the same a decade ago. However, if we wish to train a model to identify a person from the past pictures of the subject, it should learn to rely only on features that would generalize to the future and not focus merely on minimizing the train risk. We may have access to the labeled data from several time steps during the train time along with their originating time index: $t=1,\dots,T$, however we may not have access to any (un)labeled data of the future. Our objective is to find a learning algorithms that generalizes better to the (immediate) future: t=T+1.
%%
Any real world supervised machine learning algorithm trains the model on the data from the past and perform prediction in future.
Many of such tasks often involve strong temporal shift from past to future. Consequently,
the training data becomes outdated, to some extent, which signficantly constrains the ability of the underlying model
to generalize to the future. For example, predicting a person's identity from a stream of past images 
requires learning to identify those features which would generalize to the future, rather than minimizing a training risk on a black-box model. More specifically, given the labeled training data in
$t\dots, T$, our objective is to find a learning algorithm which will generalize to immediate future $t=T+1$.
 



A starting point for a model that would pick on the desired temporal patterns in our case is a model that along with the input also takes the originating time of the instance but imposes a simple Empirical Risk Minimization, denote {\ermt}. {\ermt}, however, has no control on how the concatenated time is utilized, on one extreme it could ignore the extra information and on other it could demonstrate a Mixture of Expert behaviour where the expert is gated by the time index. In the latter case, we would be learning locally optimal models for each time step without any sharing among them. On the other hand, methods have been proposed that require learning representations that are indistinguishable between the time steps~\citep{wang2020continuously,ganin2016domain}\todo{Does CDOT fit here?}, we call these collectively as erasure methods; These methods seek to learn only stable features between the time steps which also would generalize well to the future. We have one extreme with {\ermt}, a potential locally private model with no sharing and on other we have erasure methods that seek to shared features of constant signal. For some underlying true function, {\ermt}'s fit would have low bias but large variance and erasure methods would have large bias (due to their constraint on desirable features) but low variance since the final features are shared across time steps. We argue that neither of these extreme might be ideal and we could do even better if we can control how much feature sharing vs locally optimal is allowed between the time steps which would let us navigate the bias-variance trade-off for even lower MSE. We illustrate further the problem with simple thought experiments in two different settings.

Consider the case when both input (x), output (y) are binary random variables, and the train data includes three time steps. For the task of learning a classifier that predicts y from x, denote the optimal classifier at time 't' as $w_t^*$ such that the classifier is $\sigma(w_t^*x+1)$. Assume the optimal classifier is of the form $w_t=a+bt$ for some non-zero $a, b$. For this setting, {\ermt} would fit $w_t$ at each time step 't' using the corresponding train data from that time step, denote $w_t^{ERM}$. Erasure methods would try and fit a time-invariant scalar, because a time-dependent coefficient would lead to distinguishable representations, that approximates the optimal classifier at each time step as closely as possible, denote $w^{E}$. When the training data per time step is limited, the estimation noise in $w^{ERM}_t$ is of the order: $1/N$ when N is the average number of examples per time step, hence we have a case of zero bias but variance of the order 3/N. $w^E$ on the other hand incurs non-zero bias, since it learns a time-invariant coefficient, of the order of b, however, since the estimate is obtained using all the examples it is of the order: 1/3N. If we instead try the middle ground and fit $w_1+w_2t$, the bias would be zero which is better than $w^E$, and variance would be better than that of $w^{ERM}$ since there are fewer parameters for the same amount of data. Which exact form of approximation is better depends on the exact values of $N, b, a$. It can often be the case that neither of the extremes have the lowest MSE value. This motivates for the need to control the complexity of feature dependence on time. \todo[inline]{We can expand on this more analytically but when we have enough training data per time step then this setting does not motivate well.}

% In above setting, we motivated the need to control the temporal dependence of coefficients which comes is of significance when the data per time step is limited. Such a requirement on controlling temporal complexity could also arise when data per time step is surplus which we illustrate through the following setup. We consider the classification task again but when the input contains two binary random variables: $x_1, x_2$.   

% VP: Need to look beyond this

% In several real world applications, machine learning systems are deployed on data which is different from the data they have been trained on. This shift may arise because of a changed data distribution (referred to as domain drift in the literature), or a changed conditional distribution of the labels given data (i.e. task drift). Further, in most naturally arising situations, there is a continuous variable underlying this drift, the most common example of this being time. For example, for data collected from satellites, the identified features in the images would be different in different seasons. The global effects of climate change would also be visible in images collected from different time periods. This drift has several underlying temporal trends, and if a model is trained on a subset of the data and deployed to make predictions on new data it would fail to generalize well, since the input would have a different feature distribution, and the decision boundary would also have changed. Adding to this complexity is the fact that practitioners would not have access to \textit{any} data from the test time while training their models, which makes applying usual domain adaptation methods difficult. \\
In such scenarios, it is imperative that the training procedure explicitly prepares the model to do well in the future. It is important to note that the objective of interest is the performance of the model on unseen future data, even if that is achieved at the cost of performance on past data. In order to achieve this goal, the training algorithm needs to encourage the model to adjust for temporal drifts both in the data distribution and the decision boundary, and be able to generalize and extrapolate well on such shifts. To closely mimic the distributions seen in real world, we restrict the problem to be such that the drift along time is not too much, and the predictions are to be made not too far in the future. Going back to the example of satellite data, it would mean that we have access to labelled data collected over few months, and we wish to make predictions on data from the next month.   \\
There have been several attempts to tackle this problem, both from a domain adaptation perspective and a concept drift perspective. The former approaches either try to \textit{predict} how the training domains evolve as time passes, using these predictions to generate new data, or they try to find feature representations which are invariant across time \cite{lao2020continuous}, and use these features to make predictions. The problem with finding transformations or generative functions from source to target domains is that such methods often require unlabelled data from the target time step, so they differ from our setting. Further, methods which aim to learn domain invariant representations are problematic since they may be discarding valuable temporal information which is essential to making a prediction\todo{Support better. What temporal information and why they are valuable?}. There have also been attempts to model the decision boundary itself as a function of time \cite{kumagai2016learning,kumagai2017learning}, however these methods often have tight constraints \todo{Should be more specific, what constraints?} on the model used, and they haven't harnessed the power of deep learning for the problem\todo{Why would their method not work with DNNs?}. \\
\todo{Should we add some notion of fine-tuning here or will that confuse the reader?}
Since the problem involves making predictions on data which is in the immediate future, we re-frame this as a task of learning a model robust to small perturbations in time, with time being one of the features. We conjecture that such functions would need to be smooth in time, and not have abrupt shifts. However, the training data available to us is from a finite number of time steps, and it is possible to fit a function perfectly at each time step without it generalizing well. Building on this intuition, we propose a method which can learn to generalize well in time by interpolating between two training time steps with a first order Taylor expansion. This provides a certain smoothness to the learnt function, and acts as a regularizer to discourage complex functions of time. It also encourages the function to make optimal use of the temporal information to extrapolate well on future time steps. Our proposed method is also general enough to work with both regression and classification settings. In order to use the time information more effectively, we also propose a modified activation function parameterized with time.\\
Our contributions in this work are - 
\begin{itemize}
\item We present several strong baselines for the problem, comparisons with which have been missed in the past, Inc. FineTune.
\item We propose a simple training algorithm to encourage a model to learn functions which can extrapolate well in the future. We do this by supervising the first order Taylor expansion of the learnt function.
\item We propose a modification on the ReLU activation function which is time aware.
\item On several real world datasets, we make head-on comparisons of \shortname\ with others and show significant gains. We motivate and illustrate the contributions of \shortname\ through a simple setting. 
\end{itemize}
The rest of the article is organised as follows - we formalize the problem and provide a sketch of our method in section \ref{sec:Formulation}, present a brief overview of prior work in section \ref{sec:Related}, propose our method in section \ref{sec:Method}, demonstrate its empirical results in section \ref{sec:Experiments} and provide insights about it in section \ref{sec:motive}.  
% immediate future
% lots of data at each step
% Extrapolate trend
% previous attempts and where they lack!
% Robustness, extrapolation

==> NeurIPS/sections/method_old.tex <==
\label{sec:proposed}
\vspace{-2mm}
 \subsection{Overview of our problem}
\vspace{-2mm}




Our approach comprises of two parts: make the network architecture time-sensitive and impose a special loss to encourage the network to generalize to the near future.  We make the network time-sensitive by both taking time as an additional input concatenated with $\vx$, and by computing a subset of the network parameters as a function of time.  When a parameter $W_j$ of a network is made time-sensitive, then $W_j$ becomes the output of a small neural network $w_j(t|\theta_j)$ with time as input and parameters $\theta_j$. Now instead of $W_j$ we train $\theta_j$ during the end to end training. The set of $W_j$s that are made time-sensitive is part of network architecture design. We present our proposed design of a time-sensitive network architecture in Section~\ref{sec:time}.  The rest of our algorithm treats the $\theta_j$s as any other network parameters and does not impose any custom smoothing on them unlike some prior work~\cite{kumagai2017learning,mancini2019adagraph}.  However,
if we apply standard training on data from $T$ training snapshots $D^1,\ldots,D^T$, we have no guarantee that the network would generalize to samples from the $P(\vx|T+1)$ distribution.  Even if $w_j(t)$s are smooth, the rest of a large network's parameters could easily overfit on exactly the $T$ data distributions on which we impose training loss. Therefore, we propose to regularize the output of the entire network.

%
%Although capture the evolving hidden feature spaces and the decision boundary, the learn't neural network can lead to very spiky gradients with respect to time, which hurts it capabilities to generalize to a future time step. 
%In order to make sure that the function learnt attempts to capture the actual dynamics along time, 
We encourage learning functions that can be approximated linearly by regularizing the curvature of $F(\vx, t)$ along time.  We impose a loss on the first order Taylor approximation of the model output. Formally, if $\mathcal{L}(\cdot ; \cdot)$ denotes a loss metric to be minimized, our gradient interpolated loss is defined as
%\begin{equation}
%    L(F(\vx,t);y) = l(F(\vx,t),y) + %\lambda l(F(\vx,t-\delta)+\delta %\frac{dF(\vx,t-\delta)}{dt},y)
%\label{eq:GIloss}
%\end{equation}

\begin{equation}
    \mathcal{J}_{GI}(y; F(\vx,t)) = \mathcal{L}(y; F(\vx,t)) + \lambda \max_{\delta\in (-\Delta,\Delta)}\mathcal{L} \Big(y; F(\vx,t-\delta)+\delta \frac{\partial F(\vx,t-\delta)}{\partial t}\Big)
\label{eq:GIloss}
\end{equation}

Here, the first term is the usual loss for fitting $F(\vx,t)$ to $y$, while the second term is the regularizer which approximates $F(\vx,t)$ using the Taylor Expansion at $t-\delta$. 
%Note that $\delta$ can be bigger than two subsequent $t_i$. 
We choose the $\delta$ adversarially within a user-provided window $\Delta$, which we set as a task-dependent hyper-parameter. When $\delta$ is negative we are computing the logits of an instance at $t$ by extrapolating from the future $t+\delta$.  This indirectly serves to supervise the function and its gradients to near-by points.  Since our goal is to generalize only to time values within a small neighborhood of the last training time, we expect this to provide better generalization to these near future points.

% as discussed in Section \ref{sec:method:delta}. 

%The entire algorithm is described in~\ref{algo:GITrain}.

%\todo[inline]{AN: The equation below and a line about curvature regularization earlier were included to give a different view of GI using the second derivative. It seems out of place right now since we don't mention it anywhere else in the article.}
%\begin{equation}
%    l(\hat{f}(x,t)-\delta^2 d^2 %\hat{f}/dt^2, y )
% \end{equation}


\subsubsection*{Understanding GI with a synthetic setup}
We present here an analysis with a simple setup to understand how GI could be more effective in generalizing to the future compared to existing methods. Consider a dataset where the input is $d$ Boolean features i.e., $\cX \in [0,1]^d$, and output label $\cY \in [0,1]$ is binary. Assume their joint distribution factorizes as $\Pr(\vx,y|t)=\Pr(y)\prod_{r=1}^d \Pr(x_r|y,t)$ where prior class probability is independent of time and $\Pr(y)=\Pr(y|t)=1/2$, and features are conditionally independent given the class label.  Assume $\Pr(x_j|y,t)=\Pr(x_j=y|t)=p_j(t)$ where $p_j(t)$ denotes the time-varying correlation between feature $x_j$ and label $y$ at time $t$. Further, let $p_j(t)$ be defined as:
\begin{flalign*}
p_1(t) = 0.2 + 0.2t,~~~p_2(t) = 0.8 - 0.2t, ~~~~p_j(t) = 0.5 + 0.49[[t=j-3]]
% & \Pr(x_2 = y|t) = p_2\\\nonumber
% & \Pr(x_j = y|t) = \begin{cases}
%     p_3 & \text{if } t=j-3\\
%     p_4 & \text{otherwise}
% \end{cases} \\\nonumber
% & p_1, p_2,p_3, p_4 = 0.6,0.7,0.99\\
\end{flalign*}
% \begin{flalign*}
% &y \sim Bern(0.5)& \\\nonumber
% & x_1 = ys_1 + (1-y)(1-s_1); s_1\sim Bern(p_1)\\\nonumber
% & x_j = ys_j + (1-y)(1-s_j); s_j \sim \begin{cases}
%     Bern(p_1) & \text{if } t=j-2\\
%     Bern(p_2) & \text{otherwise}
% \end{cases} \\\nonumber
% & p_1, p_2 = 0.9, 0.5\\
%\end{flalign*}
Here the first three feature's correlation with class label evolves linearly with time, whereas each of the remaining features have strong correlation exactly at one time stamp, and are uninformative elsewhere. Given the conditional independence of features the following parametric form can perfectly fit the data, while allowing easy interpretation:
$$f(\mathbf{x},t) = \sum_{j=1}^d w_j(t|\theta_j) x_j + w_0(t|\theta_0)$$
where the $w_j(t|\theta_j)$ can be any neural network with input $t$ and parameters $\theta_j$.  We used a two layer network with ReLU activation of width 50 and 20 respectively.
% Note that according to the formulation mentioned, for each training time step there are two features equally predictive for the label ($x_1,x_{t+1}$). Hence, one could fit the training data well by giving a high weight to either of these features. \todo[inline]{This reasoning is incorrect. Both are useful, not either one and can jointly do better than just depending on one.}

Assume we have training data at $t=0,1,2$ and we need to deploy at $t=3$.
According to the above parameterization, the baseline ERM could fit training data well by giving a high weight to $x_3,x_4,x_5$ at times $t=0,1,2$ respectively, and low weight at other times.  There is no control on how the $w_j(t)$ values evolves with time, and there is no reason for the classifier to generalize to $t=3$.  In fact here the test accuracy is 49\% (slightly worse than random) while  the train accuracy is 99\%.  Figure~\ref{fig:simple_weights} shows the weights as a function of time (solid lines) for $w_1,w_2,w_4,w_5$ and we see that $w_2$ is largely ignored while $w_4,w_5$ take large values and have large swings.

When GI is applied on this dataset, we impose an additional loss on 
logits computed from $\sum_j x_j[w_j(t-\delta) + \delta \frac{\partial w_j(t-\delta)}{\partial t}]$.  This loss provides supervision on not just the parameter values at the training times, but also requires that their gradients be correctly oriented to allow reconstruction at near-by points.  This has the effect of smoothing the $w_j(t)$ functions for the transient features, and recovering the correct slope of the linear features.  Further, when $\delta$ is negative then for instances close to $T$ we also indirectly supervise the logits and their gradient at future times $T+\delta$.
%
Figure~\ref{fig:simple_weights} shows the weights learned by GI in contrast with those of ERM. The accuracy obtained by GI is 55.4, which is higher than that of any other model.  Without clairvoyance, and without access to even unlabeled data from $t=3$, it may be difficult to get better results in expectation over future datasets.   

Since one of the main outcomes of GI is smoothing $w_j(t)$s, a natural question is whether the benefits of GI could also be obtained by a simple regularizer on the gradient of the network with respect to time. In that context we explored an alternative gradient penalized training objective as follows:
\begin{equation}
    \mathcal{J}_{GR}(F(\vx,t);y) = \mathcal{L}(F(\vx,t);y) + \lambda \left\lVert \frac{\partial F(\vx, t)}{\partial t}\right\rVert_2^2
\label{eq:Gregloss}
\end{equation}
This objective requires us to carefully select the weight $\lambda$ of the regularizer.  If $\lambda$ is large, the objective will converge to constant $w_j(t)$. Even for weights that have a predictable linear change along time, would not be fitted well.  This would correspond to the `ERM const' numbers in the table.  For small $\lambda$, the weights would not be sufficiently smooth.  The merit of GI is that by imposing a loss on the gradient interpolated loss, we are able to supervise the correct level of smoothness based on label data. 

Methods such as CIDA that attempt to learn time-invariant representations at the last layer also do not perform well. We implement this method by making the vector $\mathbf{w}(t)*\mathbf{x}$ (where $*$ denotes element-wise product) as the time invariant representation of a data point.  A successful implementation of the adversarial loss would make the expected value of $E_{P(x_j|t)}[w_j(t) x_j]$ independent of time. In our generative model, it can be see that the marginals $E_{P(x_j|t)}[x_j]=1/2$, and thus independent of time.  This implies that an ideal classifier as per CIDA would make $w_j(t)$ a constant independent of time. When such a classifier is fit on the data, we get a train accuracy of 73\%, but test accuracy does not improve beyond random and is at 49.5\%.

The merit of GI is that it allows the last layer to change with time, and yet generalize to the immediate future.

%$L_2$ regularization - We apply $L_2$ regularization to the learnt weights $w_j(.)$.      
%We present the learnt weights as a function of time in fig: \ref{fig:simple_weights}. We can see that ERM learns to give a higher weight to the $(j+1)^{th}$ variable at time $j$. We also report the sensitivity of the label to each feature at different times in tables \ref{}. 

%Sensitivity here for each feature is defined as $P(y|x) - P(y|\tilde{x}_j,x_{-j})$ where $\tilde{x}_{j}$ indicates the value of the $j^{th}$ feature is flipped. It gives us another measure of importance for each feature. \\
% This arises because the functions fitted by these methods are agnostic to the big picture time information. Further, the network is over-parameterized, leading to it being powerful enough to capture all the information at each point... overfitting etc. \\
%In order to bias our learning algorithm towards functions which are more generalizable in time, we propose to make them aware of the relation between the data at different time steps through \textit{gradient interpolation}.   


%We present the learnt weights and the sensitivity of this loss on the simple setting in fig \ref{fig:simple_weights} and table \ref{tab:simple:gi_sens}. One can see by comparing against the learnt solution from ERM that our method learns to give higher weights to $x_1$ than the other variables, since a function learnt this way is able to interpolate better within the training times. This function also extrapolates better, as can be seen from the performance reported in table \ref{tab:simple:perf}.



% \begin{table}[htb]
%     \centering
%     \begin{tabular}{|c|c|c|c|c|}
%     \hline
%         Metric & ERM &  GI ($\delta_{max}=1$) & GI ($\delta_{max}=2$) & GI ($\delta_{max}=3$)\\\hline
%         Test Loss & 1.728 & 1.205  &1.028 & {\bf 1.004}\\\hline 
%     \end{tabular}
%     \caption{Comparison of average cross-entropy loss for different algorithms in the simple setting.}
%     \label{tab:simple:perf}
% \end{table}

% \begin{table}[htb]
%     \centering
%     \begin{tabular}{cccc}
%     \toprule

% Model & Test Accuracy & Test CE & Train Accuracy \\
% \midrule
% ERM & 0.5922 & 1.822 & 0.930 \\
% ERM with $L_2$ & 0.5294 & 0.686 & 0.667 \\
% GI & 0.6648 & 1.516 & 0.917 \\
% GI with KL & 0.6116 & 1.686 & 0.928 \\
% % CIDA & 0.6146 & 1.575 & 0.931 \\
% CIDA &  0.7886 & 0.609 & 0.904 \\
% \bottomrule
%     \end{tabular}
%     \caption{Comparison of performance for different algorithms in the simple setting.}
%     \label{tab:simple:perf}
% \end{table}


% \begin{table}[htb]
%     \centering
%     \begin{tabular}{cccc}
%     \toprule

% Model & Test Accuracy & Test CE & Train Accuracy \\
% \midrule
% ERM & 0.506 & 10.204438591003418 & 0.99 \\
% ERM\_L2 & 0.4996 & 0.7032872319221497 & 0.6506666666666667 \\
% GI & 0.5676 & 3.836525249481201 & 0.9446666666666668 \\
% CIDA & 0.6228 & 0.7552089691162109 & 0.8426666666666668 \\

% \bottomrule
%     \end{tabular}
%     \caption{Comparison of performance for different algorithms in the simple setting when first feature is linear.}
%     \label{tab:simple:perf}
% \end{table}


% \begin{table}[htb]
%     \centering
%     \begin{tabular}{cccc}
%     \toprule

% Model & Test Accuracy & Test CE & Train Accuracy \\
% \midrule

% ERM & 0.4876 & 10.613 & 0.99 \\
% ERM_L2 & 0.5552& 0.684 & 0.658 \\
% GI & 0.5902 & 3.850 & 0.942 \\
% % CIDA & 0.4968 & 4.062 & 0.988 \\
% CIDA & 0.6534 & 0.6980 & 0.792 \\

% \bottomrule
%     \end{tabular}
%     \caption{Comparison of performance for different algorithms in the simple setting when first feature is linear with slope $0.1$ and second feature is constant with $p=0.7$.}
%     \label{tab:simple:perf}
% \end{table}


% \begin{table}[htb]
%     \centering
%     \begin{tabular}{cccc}
%     \toprule

% Model & Test Accuracy & Test CE & Train Accuracy \\
% \midrule

% ERM & 48.8 & 11.6 & 99. \\
% ERM $L_2$ & 50.8 & 0.7 & 64.1 \\
% CIDA & 50.1 & 1.9 & 83.7 \\
% GI & 54.6 & 4.3 & 94.9 \\
% ERM const & 64.8 & 0.8 & 78.5 \\
% \bottomrule
%     \end{tabular}
%     \caption{Comparison of performance for different algorithms in the simple setting when first feature is linear with slope $0.15$ and second feature is constant with $p=0.7$.}
%     \label{tab:simple:perf}
% \end{table}




% Model & Test Accuracy & Test CE & Train Accuracy
% ERM & 0.5922 & 1.8228198647499085 & 0.9306666666666666
% ERM_L2 & 0.5294 & 0.6864143967628479 & 0.6679999999999999
% GI & 0.6648 & 1.5161160349845886 & 0.9179999999999999
% GI_KL & 0.6116 & 1.6861860156059265 & 0.9286666666666665
% GI_finetune & 0.6814 & 1.5763799786567687 & 0.9200000000000002
% GI_KL_finetune & 0.5838 & 1.6566529989242553 & 0.9286666666666665
% CIDA & 0.6146 & 1.5757513284683227 & 0.9319999999999998

\iffalse
\begin{table}[htb]
    \centering
    \begin{tabular}{|l|r|r|r|r|r|}\hline
        t=1 & -0.40 & 0.01 & 0.25 & 0.06 \\\hline
        t=2 & 0.58 & 0.25 & 0.00 & 0.00 \\\hline
        t=3 & 0.40 & 0.01 & 0.01 & 0.37 \\\hline
        t=4 & 0.23 & -0.01 & 0.00 & -0.01 \\\hline
    \end{tabular}
    \caption{ERM: Qualitative comparison on Simple data}
    \label{tab:simple:erm_sens}
\end{table}

\begin{table}[!htb]
    \centering
    \begin{tabular}{|l|r|r|r|r|r|}\hline
    t=1 & 0.41 & 0.01 & 0.24 & 0.04 \\\hline
    t=2 & 0.72 & 0.08 & -0.01 & -0.01 \\\hline
    t=3 & 0.52 & 0.00 & 0.01 & 0.27 \\\hline
    t=4 & 0.36 & -0.00 & 0.01 & 0.00 \\\hline
    \end{tabular}
    \caption{GI: Qualitative comparison on Simple data}
    \label{tab:simple:gi_sens}
\end{table}

% shown below are sensitivity for $\delta=3$
    % t=1 & 0.39 & 0.01 & 0.25 & 0.03 \\\hline
    % t=2 & 0.70 & 0.13 & -0.00 & -0.00 \\\hline
    % t=3 & 0.48 & 0.00 & 0.00 & 0.27 \\\hline
    % t=4 & 0.34 & -0.01 & -0.00 & -0.01 \\\hline

% shown below are sensitivity for $\delta=2$
% 0.40 & 0.01 & 0.24 & 0.04
% 0.71 & 0.09 & -0.01 & -0.01
% 0.50 & 0.00 & 0.01 & 0.28
% 0.31 & -0.00 & 0.01 & 0.00
\fi


\begin{figure}[htb]
  \centering
    \begin{minipage}{0.4\linewidth}
    \centering
    \begin{tabular}{|l|c|c|}
    \hline
    Model & Test & Train \\
    \hline
    ERM & 48.8 & {\bf 98.9} \\
    CIDA & 49.5  & 73.3 \\
    ERM const & 47.4 & 75.1 \\
    GradReg & 49.1  & 77.0 \\
    GI & {\bf 55.4}  & 95.0 \\
    %GI_finetune & 50.5 & 7.3 & 97.6 \\
    % GI_finetune_delta_3 & 0.5509999999999999 & 5.463326644897461 & 0.9206666666666667
    % ERM const & 0.4856 & 4.580 & 0.842 \\
    % ERM & 0.4876 & 10.347 & 0.9886 \\
    % GI & 0.5264 & 4.347 & 0.9413 \\
    % CIDA & 0.4966 & 1.442 & 0.79 \\
    \hline
    \end{tabular}
    % \captionsetup{justification=centering}
    \captionof{table}{Comparison of accuracy for different algorithms in the simple setting.}
    \label{tab:simple:perf}    
    \end{minipage}\hfill
    \begin{minipage}{0.6\linewidth}
% \begin{figure}[!tbp]
  \centering
%   \captionsetupfigure}
  %\subfloat[$p_1$,$p_2$ both linear]
  %{\includegraphics[width=0.5\textwidth]{ehre/figures/Normalized_Simple_withGT.png}\label{fig:f1}}
%   \hfill
      \includegraphics[width=1.0\textwidth]{ehre/figures/Simple_weights.pdf}
      \captionof{figure}{Weights learnt as a function of time}
      \label{fig:simple_weights}
  % \end{figure}    
    \end{minipage}

\end{figure}




\iffalse
\begin{table}[!htb]
    \centering
    \begin{tabular}{|l|r|r|r|r|}\hline

\hline ERM & & & & \\ coeff 1 & 0.159 & 0.197 & 0.222 & 0.170 \\ coeff 2 & 0.039 & 0.074 & 0.099 & 0.028 \\ coeff 3 & 0.090 & 0.935 & 0.213 & 0.014 \\ coeff 4 & 0.982 & 0.235 & -0.147 & -0.116 \\ coeff 5 & -0.006 & -0.164 & 0.935 & 0.978 \\
\hline GI finetune & & & & \\ coeff 1 & 0.012 & 0.054 & 0.120 & 0.110 \\ coeff 2 & 0.031 & 0.068 & 0.086 & 0.054 \\ coeff 3 & 0.018 & 0.818 & 0.373 & 0.038 \\ coeff 4 & 0.997 & 0.512 & -0.018 & -0.042 \\ coeff 5 & 0.063 & 0.249 & 0.916 & 0.991 \\
\hline GI & & & & \\ coeff 1 & -0.061 & 0.090 & 0.232 & 0.239 \\ coeff 2 & 0.114 & 0.128 & 0.037 & -0.028 \\ coeff 3 & 0.448 & 0.776 & 0.453 & 0.166 \\ coeff 4 & 0.879 & 0.478 & -0.232 & -0.543 \\ coeff 5 & -0.097 & 0.379 & 0.828 & 0.787 \\
\hline CIDA & & & & \\ coeff 1 & 0.042 & 0.051 & 0.042 & 0.035 \\ coeff 2 & 0.053 & 0.271 & 0.036 & -0.050 \\ coeff 3 & 0.449 & 0.606 & 0.462 & 0.355 \\ coeff 4 & 0.720 & 0.433 & 0.715 & 0.824 \\ coeff 5 & 0.525 & 0.608 & 0.522 & 0.437 \\
\hline Ground Truth & & & & \\ coeff 1 & -0.086 & 0.044 & 0.181 & 0.845 \\ coeff 2 & 0.181 & 0.044 & -0.086 & -0.535 \\ coeff 3 & 0.000 & 0.998 & 0.000 & 0.000 \\ coeff 4 & 0.980 & 0.000 & 0.000 & 0.000 \\ coeff 5 & -0.000 & 0.000 & 0.980 & 0.000 \\
\end{tabular}
\caption{Normalized Weights for different algorithms at t=0,1,2,3}
\end{table}
\fi
% \begin{figure}[!tbp]
%   \centering
%   \begin{subfigure}
%   \includegraphics[width=0.4\textwidth]{ehre/figures/ERM_Simple.png}\label{fig:simple:erm_weights}
%   \caption{ERM}
%  \end{subfigure}
%   \begin{subfigure}
%   \includegraphics[width=0.4\textwidth]{ehre/figures/Gi_Simple.png}\label{fig:simple:erm_weights}
%   \caption{GI}
%  \end{subfigure}
%   \caption{Weights learnt as a function of time}
% \end{figure}
% Make two points together - ERM can fit perfectly without extrapolating?
% Picks up less variable functions?
% How do we talk about complexity of functions?

\subsection{Time-sensitive Model Architecture}
\label{sec:time}
\todo[inline]{This section requires a careful look. Many symbols are not defined.  Someone please clean this up.}
\subsubsection{Time Vectorization}
A naive way to force time-dependence to a neural network's predictions is to include time as a feature to our training data. Formally speaking, if $(x, y) \in \mathcal{D}^t$ is a point in our training data, then we obtain an augmented feature vector $[x, t]$ where $[. , .]$ denotes a concatenation. 

In order to capture more complex temporal trends including periodicity in the data along time, we also encode each time $t$ using a learnable $k$-dimensional vector representation $\tau(t)$ as discussed in \cite{kazemi2019time2vec}. The $i^{th}$ component of this vector is computed as - 
\begin{equation}
    \mathbf{\tau}_i(t) = \begin{cases}
w_it + b_i, \  1 \geq i \geq m\\
\mathcal{H}(w_it + b_i), m < i \leq k\\
\end{cases}
\end{equation}
where $dim(\tau) = k$, $w_i$ and $b_i$ are weights and biases associated with the $i^{th}$ component of $\tau$, and $\mathcal{H}(.)$ is a periodic function, like $sin (.)$. Since we use the same vector representation of time across the entire model, training of an additional $k$ parameters is required.

\subsubsection{Temporal ReLU}
One way to capture the time-evolving nature of the data distribution is to model the parameters in a time dependent fashion. Previous works have tried to do this by modelling the weights of a linear classifier as a Gaussian Process \cite{kumagai2017learning}, or modelling the batch normalization parameters of a neural network through a kernel regression \cite{mancini2019adagraph}. We argue that extending the former approach to a deep network will be computationally infeasible.

We hence propose to make the activation function of a neural network time dependent by introducing the leaky Temporal ReLU function as shown below. 
\todo[inline]{VP: This formulation of TReLU needs a better motivation. Why only change the function on one side of the relu function? Why is this a general form that can capture the desired functions of time? Is this h(t), f(t) shared among all ReLU?}
\begin{equation}
    TReLU(\mathbf{x},t) = \begin{cases}
\mathbf{x}, \  \vx \geq g(t)\\
h(t)(\vx-g(t)) + f(t), \ \vx < g(t)\\
\end{cases}
\end{equation}
Here, $h,f$ are shallow neural networks  which aim to learn the threshold and slope parameters. In our experiments we use a bottleneck neural network with $1$ hidden layer, an input dimension of $dim(\mathbf{t})$, a hidden size of $1$, and an output dimension of $dim(\mathbf{x})$. \\
% The intuition behind using this activation function is to capture the subspace shift in a neural network...

We find that combining the Temporal ReLU with time vectorization is a powerful way to capture evolving subspaces. As we show in the appendix, a small two-layer neural network with these techniques can capture a decision boundary which translates or rotates as time progresses.
\todo[inline]{VP: Are all ReLUs changed to TReLUs? Do we get gains as good also when transforming only the last layer ReLUs? For a model with `r' relus transformed to trelu, how many parameters are being added?}



\todo[inline]{Algorithm below needs to be cleaned up with respect to the notations used in the paper.}
\begin{algorithm}[htbp]
   \caption{Training with Gradient Interpolation}
   \label{algo:GITrain}
\begin{algorithmic}
%   \STATE {\bfseries Input:} $X\in \R^{d\times m}$ and $H_1, ..., H_d\in\R^{d\times d}$. 
%   \STATE {\bfseries Output:} $A_{1}=P_1\cdots P_{d/m} X=H_1 \cdots H_d  X$. 
   \STATE
   \STATE // Step 1 - Pre-train $F(\vx,t)$ over the entire dataset
   \FOR {$i=0$ {\bfseries to} $t$}
   \STATE {Minimize $\mathcal{L}(F(\vx,i),y)$ for all datapoints in domain $i$ }
   \ENDFOR
   \STATE
   \STATE // Step 2 - Finetune $F$ using Gradient interpolation 
   \FOR{$i=0$ {\bfseries to} $t$}
   \FOR{$x,y$ {\bfseries in} $D^i$}
   \STATE // Compute $\delta$ adversarially over $k$ steps
   \STATE $\delta \sim Unif(-\delta_{max},\delta_{max})$ \hfill \textit{Sample $\delta$ randomly}
   \FOR{$j=0$ {\bfseries to} $k$}
   \STATE Approximate $F_{GI}(\vx,i)$ as $F(\vx,i-\delta) + \delta \frac{\partial F(\vx,i-\delta)}{\partial t} $
   \STATE Compute $\mathcal{L}(F_{GI}(\vx,i),y)$
   \STATE $\delta := \delta + \eta \frac{\partial{l}}{\partial{\delta}}$ \hfill \textit{Maximize $l$ w.r.t. $\delta$}
   \ENDFOR   
   \STATE Clamp $\delta$ in $[-\delta_{max}, \delta_{max}]$
   \STATE Optimize equation \ref{eq:GIloss} using the obtained $\delta$
   \ENDFOR
   \ENDFOR
   \STATE \textbf{return} $F(.,.)$. 
\end{algorithmic}
\end{algorithm}

% \todo{ST: Changed the algorithm to include clamping}

\subsection{Overall Algorithm}
\todo[inline]{Rewrite this section to read like description of the overall alg}
% We note that the second term in equation \ref{eq:GIloss} computes the Taylor expansion at time $t-\delta$ while neglecting the higher order terms. Hence, for a small enough $\delta$, this value should be close to $\hat{f}(x,t)$. However, we are interested in ensuring that the function is smooth to perturbations in time, and generalizes to the future time-stamp $t_{T+1}$.  
The second term in the loss~\eqref{eq:GIloss} does not add any new information when $\delta$ is zero. It adds more information when the linear approximation is bad, i.e. when distance between the true and interpolated term% $\|\hat{f}(x, t) - \hat{f}(x, t-\delta) - \delta \frac{\partial f(x, t-\delta)}{\partial t}\|$
%
is large. When $\delta$ is very large on the other hand, we would be approximating the prediction at 't' from a distant past. Such large jumps for gradient interpolation could encourage the network to not utilize 't' at all for prediction. We would, thereby, cap the maximum value of $\delta$, to say $\delta_{max}$. We obtain $\delta$ that leads to the worst linear approximation through an implicit loss term shown in the inner most loop of the Alg~\ref{algo:GITrain}.
Hence adversarially select a $\delta$ to maximize the loss and then optimize $\hat{f}$ using this $\delta$. We clamp the value of $\delta$ to ensure that it does not grow unbounded. This value of $\delta_{max}$ also acts as a tradeoff between interpolating across multiple time steps while sacrificing train accuracy and learning models which are completely disconnected across time but have high train accuracies.  \\
In order to make this optimization faster, we choose a single delta per minibatch of examples, and use a warm start by initializing the delta to the value from the previous minibatch. We find that this leads to a significantly faster run time while not compromising much with the accuracy, as reported in table ().

% \subsection{Optimization of $\delta$}
% The second term in the loss~\eqref{eq:GIloss} does not add any new information when $\delta$ is zero. It adds more information when the linear approximation is bad, i.e. when distance between the true and interpolated term% $\|\hat{f}(x, t) - \hat{f}(x, t-\delta) - \delta \frac{\partial f(x, t-\delta)}{\partial t}\|$
% is large. When $\delta$ is very large on the other hand, we would be approximating the prediction at 't' from a distant past. Such large jumps for gradient interpolation could encourage the network to not utilize 't' at all for prediction. We would, thereby, cap the maximum value of $\delta$, to say $\delta_{max}$. We obtain $\delta$ that leads to the worst linear approximation through an implicit loss term shown in the inner most loop of the Alg~\ref{algo:GITrain}. A more explicit objective would be to directly maximize the approximation error as shown below. \todo{VP: Can we check if what we are doing now and $\delta$ obtained by below eqn. are equivalent? \\}

% \begin{equation}
% \delta^* = \max_{\textcolor{blue}{-\delta_{max}}\leq\delta\leq\delta_{max}} \|\hat{f}(x, t-\delta) + \delta\frac{\partial \textcolor{blue}{\hat{f}} }{\partial t} - \hat{f}(x, t)\|^2    
% \label{eqn:delta}
% \end{equation}

% The equation above can be rewritten in the more familiar form from adversarial training literature if we cast it as search in the neighbourhood of the original instance that maximizes certain loss. An equivalent objective is shown below. \todo{AN - This only holds if $\delta$ is allowed to be negative?}

% \begin{equation}
%     t^* = \max_{L_1(t, t^*)\leq\delta_{max}}\|\hat{f}(x, t^*) + (t-t^*)\frac{\partial \textcolor{blue}{\hat{f}} }{\partial t} - \hat{f}(x, t)\|^2
% \label{eqn:adv_delta}
% \end{equation}


% \textbf{Why the two objectives may not be equivalent} - \\
% For a regression case, let $g(\delta) = \hat{f}(x, t-\delta) + \delta\frac{\partial \textcolor{blue}{\hat{f}} }{\partial t} - \hat{f}(x, t) $ and $c = \hat{f}(x, t) - y$. Then eq\ref{eqn:delta} can be rewritten as
% \begin{equation}
%     \delta^* = \max_{\textcolor{blue}{-\delta_{max}}\leq\delta\leq\delta_{max}} \|g(\delta)\|^2    
% \end{equation}
% Whereas currently the inner loop in Alg \ref{algo:GITrain} computes $\delta$ as 
% \begin{equation}
%     \delta^* = \max_{\textcolor{blue}{-\delta_{max}}\leq\delta\leq\delta_{max}} \|g(\delta) + c\|^2    
% \end{equation}
% In order to see why the two aren't equivalent, consider $g(\delta) = \delta^2-5$ and $c=4$, with $\delta$ bounded between $[0,2]$. Then, $\delta^*$ from eq\ref{eqn:delta} gives 0, while 
% The objectives in Eqns~\eqref{eqn:delta},~\eqref{eqn:adv_delta} are equivalent but obtaining $t^*$ directly by maximizing eqn:~\eqref{eqn:adv_delta} would find a better solution since we would be invoking $\frac{\partial f}{\partial t}$ multiple times and not just solve for best jump using single gradient direction obtained from $\frac{\partial f(x, t-\delta)}{\partial t}$ in eqn:~\ref{eqn:delta}.

==> NeurIPS/sections/outline.tex <==
\section*{Outline*}

What is our main story?

List of sections and outline
\begin{enumerate}
    \item Introduction - Introducing the problem, why it is difficult, our simple insight of regularizing, list contributions
    \item Related Work? - Survey previous settings and put works on continuous adaptation. Also put smoothness and generalization works? Our narrative here could be?
    \textcolor{blue}{[Our lit. review here should primarily be on works related to continuous/predictive domain adaptation. This includes mostky work done during seminar phase and additional papers that came out later. Also must include all works that we compare our results to. Maybe Optimal Transport Works?]}
    \item Setting - Emphasize on zero shot nature of problem.
    \textcolor{blue}{Emphasize on the data distribution shifts that inspires us to take this approach. Extend any related discussion from Introduction here. [I would suggest we have a separate section for the setting if it's detailed enough?]}
    \item Our Approach - 

    \begin{enumerate}

        \item Time Vectorization
        \item TReLU - Motivating example of translating domains/rotating domains? Introduce the math/formal notations of our method
        \item Gradient Interpolation - Provide intuition of smoothness for robustness to adversarial attack/generalization. Write out our formal equations. Provide Taylor expansion intuition? Make point that algo won't work without architectural innovations? \\
        \textbf{Adversarial Delta} Emphasize batchwise delta selection with intuition.
        % \item Ordinal classifier? \textcolor{blue}{This I am not quite sure. What is the motivation behind including that?}
    \end{enumerate}
    \item Experiments - 
    \begin{enumerate}
        \item Introduce baselines and previous works
        \item Introduce datasets.
        \item Two moons
        \item MNIST - Describe architecture? What story?
        \item Medical -
        % Ordinal did better, should we include? \textcolor{blue}{I think we just ignore the existence of Ordinal Classifier in our work :p} 
        \item Housing - Ours did better than unlabelled CIDA also.
        \item General point - we can show that our baselines were boosted with TReLU and T2Vec to show its effectiveness. This could also be a comparison if we decide to incorporate these into CIDA/CDOT. Make sure that the number of parameters are consistent! 
        \item More? \textcolor{blue}{M5. Also some other image data used in past papers was in my mind. But lets consolidate all these first.}
    \end{enumerate}
    \item Qualitative/Mathematical Analysis
    \begin{enumerate}
        \item With two moons and housing we can show gradient diagrams, and more defined decision boundaries
        \item What other interesting things can we show? \textcolor{blue}{[We can include some illustration of how the choice of TReLU and time vectorization helps in the decision boundary]}. We can also show how $\delta$ changes in the adversarially chosen manner for different datasets, i.e. it is not always on the clamping boundary. 
        \item Ablations - Use only TReLU without GI(our baselines). Use a fixed $\delta$. Use only GI without TReLU by making time a feature.
        \item Mathematical bounds if possible
    \end{enumerate}
\end{enumerate}


Listing out our contributions
\begin{enumerate}
    \item Architectural - We introduce a time dependent non-linearity which is effective in capturing evolving domains.   
    \item Algorithmic - We provide a simple algorithm to regularize our model to smoother functions which is surprisingly adept at generalizing to unseen domains. (Should we also include our ordinal classifier approach?)  
    % \item Analysis - Do we include any bounds here? How about simple analysis for the TReLU? \textcolor{blue}{This can be included in the qualitative analysis section}
\end{enumerate}


==> NeurIPS/sections/related.tex <==
Numerous approaches have been taken to tackle these issues. Transformation based approaches~\cite{courty2016optimal,gong2012geodesic} try to find a function that maps data from the past into the target time. 

%These methods assume that data from all domains are available. These also do not have the temporal assumption that the domains are changing continuously over time. As a result, these methods work well for a fixed source and a fixed target domain. 

\cite{courty2016optimal} uses a Optimal Transport to find a map between the source and the target domain, then transforming samples from the source to the target. A classifier is learnt on these transformed samples. \cite{gong2012geodesic} projects the data of the source and the target domains to a subspace that "best" represents both the domains. Then they develop a kernel function called Geodesic Flow Kernel (GFK) to to find an inner product between these projections, which they subsequently use to train a kernel-based classifier.

Variations to these transformation based methods have been made to adapt to situations in which the domains change continuously. These include ~\cite{jimenez2019cdot} and ~\cite{hoffman2014continuous} which deal with domains that continually change with time. \cite{jimenez2019cdot} propose \textit{CDOT}, which applies optimal transport  with a regularization to take into account the similarity between the maps of 2 successive domains. \cite{hoffman2014continuous} modifies to work in an environment where the target data is given as a stream, which is continually changing.


Another approach taken by many research works is to treat the decision function itself as non-stationary. These approaches are useful when the task changes, but not necessarily the data, over a period of time. 

Multiple works target this problem. \cite{mancini2019adagraph} uses deep-neural networks which have some domain-specific and domain-generic parameters. The domain-specific parameters have an additional constraint that takes into account the similarity between domains. These similarities  are represented by a graph structure.

Other methods like ~\cite{kumagai2016learning} and \cite{kumagai2017learning} consider only a logistic regression classifier, but its parameters are functions of time. They model the parameters as stochastic processes like vector autoregression (VAR) and Gaussian process. 

Domain Adversarial methods like CIDA~\cite{wang2020continuously} and DANN~\cite{ganin2016domain} have obtained state of the art results in continuous domain adaptation tasks. CIDA proposes to find a domain invariant encoding for all available source data which is used to make the final prediction. These encodings are learnt adversarially with the help of a domain discriminator which takes an encoding and identifies which domain the actual data may belong to.

Online learning methods such as FTPL and FTRL~\cite{suggala2020follow} could also provide an alternate approach to the problem. However, the evaluation schema of such methods is usually different from our setting. 


The methods discussed so far which consider a non-stationary decision boundary optimize their models by maximizing the likelihood on the source data. This is non-intuitive in tasks requiring training for the future, as we are interested in forecasting only future data which have a different distribution. The transformation based methods however consider that the target data is either known, or it arrives as a stream, in which case periodic updating the model is possible. None of these methods provide a solution to the case where the future data is completely hidden, and the prediction model not needing any retraining after future data appears. The question arises how is it possible to modify the training objective to consider only the future domain.

The rest of the article is organized as follows. First we define our problem more formally in Section 3. We describe in detail our Gradient Interpolation algorithm and other tricks like Time vectorization and Temporal activation functions in Section 4. Our experimental results are detailed in Section 5.

Discuss this paper:
Learning Dynamics of Decision Boundaries without Additional Labeled Data https://dl.acm.org/doi/abs/10.1145/3219819.3219967

==> NeurIPS/sections/setup.tex <==
\noindent

In this section, we introduce the discuss in detail about out problem setting. We first introduce the notion of a \textit{domain} and a \textit{task}. A \textit{domain} $D$ uniquely identified by $u$ is composed of a $d$-dimensional feature space $\mathcal{X} \subset \mathbb{R}^d$ having a marginal probability distribution of $P(\mathbf{X})$. A task $T$ has label space $\mathcal{Y}$ and a conditional probability distribution $P(\mathbf{Y}|\mathbf{X})$. $\mathbf{X}$ and $\mathbf{Y}$ are random variables.~\cite{}

Traditional prediction problems in machine learning assume that the training data $\mathbf{X_{tr}}$ and the target data $\mathbf{X_{ts}}$ are sampled from the same distribution $P(\mathbf{X})$. This assumption does not hold 

\noindent
\textbf{Training for the future:}
\todo[inline]{We should perhaps use $t_i$ instead of $u_i$ to make it clear that we are primarily thinking about time.}
Formally defining our setup, we have $T$ source domains $\mathcal{D}^1, \mathcal{D}^2, ... \mathcal{D}^T$ for which we have labelled data $(\mathbf{X}^i, \mathbf{Y}^i) \in \mathcal{D}^i$ $\forall i \in [1, T]$. The source domain $\mathcal{D}^i$ is uniquely identified by $u_i$. 
We assume that there is an ordering on $u_i$'s, i.e. $u_1 \leq_R u_2 ... \leq_R u_T$ where $\leq_R$ is some ordering relation. 
We have a target domain $(\mathbf{X}^{T+1}, \mathbf{Y}^{T+1}) \in \mathcal{D}^{T+1}$ with domain information $u_{T+1}$ for which we do not have any labelled or unlabelled data during training. \textcolor{blue}{[Comment: What about $T+\delta$ instead of $T+1$ ?]} Our objective is to learn the true distribution $P(\mathbf{Y}^{T+1} | \mathbf{X}^{T+1} | u_{T+1})$

Further we assume that the \textit{domain} and the \textit{task} are conditioned on the domain identifier $u$, i.e.; our data distribution takes the form of $P(\mathbf{X} | u)$ and the label distribution $P(\mathbf{Y} | \mathbf{X}, u)$ The task at hand is to fit the $P(\mathbf{Y}^T | \mathbf{X}^{T+1}, u_{T+1})$, i.e. the conditional probability of the labels on the target domain given only the $T$ source domains discussed earlier. We make no assumption on the nature of the distributions. %We do not bother about maximizing $P(\mathbf{Y}^i | \mathbf{X}^i, t_i)$ for $i = 1, ... \tau$ source domains. From here onwards, we use "time" and "domain information" interchangeably although domain information need not always be time. 

The joint distribution of the input and labels $P(\mathbf{X}, \mathbf{Y} | u)$ changes along domains due to 2 reasons - The marginal distribution of the data of 2 domains may not be same, i.e. $P(\mathbf{X} | u_s) \neq P(\mathbf{X} | u_t)$ for $u_s \neq u_t$. This is known as \textit{domain shift}. Also, the conditional distribution of labels given the input may change with domains, i.e. $P(\mathbf{Y}|\mathbf{X}, u_s) \neq P(\mathbf{Y^t}|\mathbf{X^t}, u_t)$ when $u_s \neq u_t$. When this happens, we say that there is a \textit{task shift}. In our problem of  training for the future, we try to tackle both of these issues.\todo{VP: Are both problems handled?}

The task and domain shifts along with the fact that we have no data from $\mathcal{D}^{T+1}$ gives a zero-shot learning. However, by observing the distribution shifts between domains, it is possible to capture the time-varying nature of both the domain and the task.



==> NeurIPS/sections/toy.tex <==
In this section, we briefly introduce our method of Gradient Interpolation and motivate and highlight the shortcomings of existing methods using a simple data setting. We first formally introduce the notion of a \textit{domain} and a \textit{task}. A \textit{domain} $D$ uniquely identified by $u$ is composed of a $d$-dimensional feature space $\mathcal{X} \subset \mathbb{R}^d$ having a marginal probability distribution of $P(\mathbf{X})$. A task $T$ has label space $\mathcal{Y}$ and a conditional probability distribution $P(\mathbf{Y}|\mathbf{X})$. $\mathbf{X}$ and $\mathbf{Y}$ are random variables.~\cite{}

Traditional prediction problems in machine learning assume that the training data $\mathbf{X_{tr}}$ and the target data $\mathbf{X_{ts}}$ are sampled from the same distribution $P(\mathbf{X})$. This assumption does not hold 

\noindent
\subsection{Training for the future:}
\todo[inline]{We should perhaps use $t_i$ instead of $u_i$ to make it clear that we are primarily thinking about time.\\
ST: Since we are using age as a domain index in sleep, I kept it this way.}

Formally defining our setup, we have $T$ source domains $\mathcal{D}^1, \mathcal{D}^2, ... \mathcal{D}^T$ for which we have labelled data $(\mathbf{X}^i, \mathbf{Y}^i) \in \mathcal{D}^i$ $\forall i \in [1, T]$. The source domain $\mathcal{D}^i$ is uniquely identified by $u_i$. 
We assume that there is an ordering on $u_i$'s, i.e. $u_1 \leq_R u_2 ... \leq_R u_T$ where $\leq_R$ is some ordering relation. 
We have a target domain $(\mathbf{X}^{T+1}, \mathbf{Y}^{T+1}) \in \mathcal{D}^{T+1}$ with domain information $u_{T+1}$ for which we do not have any labelled or unlabelled data during training. \todo{What about $T+\delta$ instead of $T+1$ ?} Our objective is to learn the true distribution $P(\mathbf{Y}^{T+1} | \mathbf{X}^{T+1} | u_{T+1})$

Further we assume that the \textit{domain} and the \textit{task} are conditioned on the domain identifier $u$, i.e.; our data distribution takes the form of $P(\mathbf{X} | u)$ and the label distribution $P(\mathbf{Y} | \mathbf{X}, u)$ The task at hand is to fit the $P(\mathbf{Y}^T | \mathbf{X}^{T+1}, u_{T+1})$, i.e. the conditional probability of the labels on the target domain given only the $T$ source domains discussed earlier. We make no assumption on the nature of the distributions. %We do not bother about maximizing $P(\mathbf{Y}^i | \mathbf{X}^i, t_i)$ for $i = 1, ... \tau$ source domains. From here onwards, we use "time" and "domain information" interchangeably although domain information need not always be time. 

The joint distribution of the input and labels $P(\mathbf{X}, \mathbf{Y} | u)$ changes along domains due to 2 reasons - The marginal distribution of the data of 2 domains may not be same, i.e. $P(\mathbf{X} | u_s) \neq P(\mathbf{X} | u_t)$ for $u_s \neq u_t$. This is known as \textit{domain shift}. Also, the conditional distribution of labels given the input may change with domains, i.e. $P(\mathbf{Y}|\mathbf{X}, u_s) \neq P(\mathbf{Y^t}|\mathbf{X^t}, u_t)$ when $u_s \neq u_t$. When this happens, we say that there is a \textit{task shift}. In our problem of  training for the future, we try to tackle both of these issues.\todo{VP: Are both problems handled?}

The task and domain shifts along with the fact that we have no data from $\mathcal{D}^{T+1}$ gives a zero-shot learning. However, by observing the distribution shifts between domains, it is possible to capture the time-varying nature of both the domain and the task.



\subsection{Motivating Example}

Consider the task of predicting binary label from a five dimensional feature vector. The training data constitutes of data from three time steps t=1, 2, 3. The generative model on features given its label and time step 't' is shown below. 

\begin{flalign*}
&y \sim Bern(0.5)& \\\nonumber
& x_1 = ys_1 + (1-y)(1-s_1) ; s_1\sim Bern(\min(1, p_1+0.1*t))& \\\nonumber
& x_2 = ys_2 + (1-y)(1-s_2); s_2\sim Bern(p_2)\\\nonumber
& x_3 = ys_3 + (1-y)(1-s_3); s_3 \sim \begin{cases}
    Bern(p_3) & \text{if } t=2\\
    Bern(p_4) & \text{otherwise}
\end{cases} \\\nonumber
& x_4 = ys_4 + (1-y)(1-s_4); s_4 \sim \begin{cases}
    Bern(p_3) & \text{if } t=1\\
    Bern(p_4) & \text{otherwise}
\end{cases} \\\nonumber
& x_5 = ys_5 + (1-y)(1-s_5); s_5 \sim \begin{cases}
    Bern(p_3) & \text{if } t=3\\
    Bern(p_4) & \text{otherwise}
\end{cases}\\\nonumber
& p_1, p_2, p_3, p_4 = 0.6, 0.7, 1.0, 0.5\\
\end{flalign*}
\todo[inline]{DE is not ignoring x1 enough.  Perhaps we could increase p2 to 0.8 so x2 looks more attractive?}
The first feature, $x_1$, has time-varying correlation with the label: 0.6, 0.7, 0.8. The second feature's label correlation does not change with time. The correlation of the subsequent features: $x_3, x_4, x_5$ is time dependent and none of the features have a clear label correlation pattern with time. I.e. there is not enough information to be able to guess the correlation of any of these features on a new time step, t=4 onward. Even if a label correlation pattern on any of the last three features exists, it is non-linear with time.  
Note that all the features have an average correlation of 0.7 during the train time. 

{\bf Optimal solution for the future:} Since the correlation of the last three features with the label is unpredictable, the optimal solution would refrain from making predictions using them. The first two feature's are promising and predictable even for the future time steps. For this reason, an optimal classifier would rely only on the first two features and ignore the rest.  

We will now compare the solutions obtained by different baselines on this dataset with 100 examples per time step and a sufficiently large backbone network (a linear layer of width 50, relu and a softmax layer). In all the baselines, we concatenate the time step of the input along with the five features making it a six dimensional vector. We make comparisons both qualitatively and empirically. All the performance numbers are obtained by averaging on 15 seed runs and when trained for 1000 epochs.

We report cross-entropy loss on a test set corresponding to future unseen time step: 4 with 0 label correlation on the last three features and the first two features generated as shown in the equation block above but with t=4. These results are shown in Table~\ref{tab:simple:empirical}. Best results are obtained when using GI or GIv3 algorithm. 

We make a qualitative comparison by reporting the sensitivity of probability of the right class wrt each of the feature. I.e. we compute the sensitivity of $j^{th}$ feature of an input $x$ with true label y as $P(y|x) - P(y|\tilde{x}_j,x_{-j})$ where $\tilde{x}_{j}$ indicates the value of the $j^{th}$ feature is flipped. 
% \todo[inline]{Wouldn't sensitivity of logit to change of that feature be more appropriate here? VP: I looked at gradients wrt inputs in order to compute this but they are noisy and unstable to look at. You have other ways of computing sensitivity? Since the features are binary, for each instance you could just calculate the difference between $\log Pr(y|x)$ with $x_j=1$ and $x_j=0$ while keeping other features unchanged. VP: Done.} 
% Pearson correlation coefficient between each feature and the computed logit using each of the algorithm for each of the time step. 
The coefficients for the five dimensional input for each algorithm is shown in Tables~\ref{tab:simple:erm},~\ref{tab:simple:de},~\ref{tab:simple:gi},~\ref{tab:simple:giv3} respectively for ERM, Domain Erasure (DI)\cite{Ganin15}, Gradient Interpolation (GI), a variant on Gradient Interpolation (GIv3). The first three rows are train data and the last is (unseen) test. 

Notice from Table~\ref{tab:simple:erm}, ERM  learns to pick a feature with highest correlation for each time step. Although, such a strategy works well to reduce the train loss, it cannot extrapolate well to the future. This is evident from its high CE loss on test and the feature correlation for t=4. Learning domain invariant representations, Table~\ref{tab:simple:de}, is better than ERM in that they reduce the dependence on the last three features. However, DI is still inferior since it under-utilizes the first feature in comparison to the second feature despite the fact that both the features have the same net correlation during the train time and first feature is more useful in the future; This is due to domain invariance constraint of the algorithm. GI, GIv3 on the other hand shown in Table~\ref{tab:simple:gi},~\ref{tab:simple:giv3} resp. both suppress the dependence on the last three features and effectively utilize the first two features. Moreover, they are least surprised by the future data which is evident from the comparable feature correlation between t=3 and t=4 in Tables~\ref{tab:simple:gi},~\ref{tab:simple:giv3}. 

GIv3 is a variant on GI in order to make it more intuitive. In GIv3, we obtain linear approximation as $\hat{f}(x, t-\delta) + \delta*\Delta f$, where $\Delta f$ is a trainable parameter. I.e. we allow for $\hat{f}(x, t)$ to change with time as long as the change is linearly predictable. GIv3 has similar performance to GI in the simple setting.

\begin{table}[htb]
    \centering
    \begin{tabular}{|c|c|c|c|}
    \hline
         ERM & DE & GI & GIv3  \\\hline
         5.86 & 2.72 & {\bf 1.15} & {\bf 1.14} \\\hline 
    \end{tabular}
    \caption{Comparison of average cross-entropy loss for different algorithms in the simple setting.}
    \label{tab:simple:empirical}
\end{table}

\begin{table}[htb]
    \centering
    \begin{tabular}{|l|r|r|r|r|r|}\hline
        t=1 & -0.00 & 0.00 & 0.00 & 1.00 & 0.00 \\\hline
        t=2 & 0.00 & 0.00 & 0.99 & 0.00 & 0.00 \\\hline
        t=3 & 0.00 & 0.00 & 0.00 & 0.00 & 0.99 \\\hline
        t=4 & 0.03 & 0.02 & -0.03 & -0.00 & -0.02 \\\hline
    \end{tabular}
    \caption{ERM: Qualitative comparison on Simple data}
    \label{tab:simple:erm}
\end{table}

\begin{table}[htb]
    \centering
    \begin{tabular}{|l|r|r|r|r|r|}\hline
    t=1 & 0.00 & 0.02 & -0.00 & 0.90 & 0.01 \\\hline
    t=2 & 0.08 & 0.07 & 0.71 & 0.00 & 0.02 \\\hline
    t=3 & 0.10 & 0.09 & 0.07 & 0.02 & 0.62 \\\hline
    t=4 & 0.11 & 0.07 & -0.01 & -0.00 & -0.00 \\\hline
    \end{tabular}
    \caption{DI: Qualitative comparison on Simple data}
    \label{tab:simple:de}
\end{table}

\begin{table}[htb]
    \centering
    \begin{tabular}{|l|r|r|r|r|r|}\hline
    t=1 & 0.02 & 0.08 & 0.02 & 0.71 & 0.04 \\\hline
    t=2 & 0.05 & 0.05 & 0.73 & 0.02 & 0.01 \\\hline
    t=3 & 0.17 & 0.15 & 0.11 & 0.04 & 0.48 \\\hline
    t=4 & 0.17 & 0.09 & -0.00 & -0.01 & 0.01 \\\hline
    \end{tabular}
    \caption{GI: Qualitative comparison on Simple data}
    \label{tab:simple:gi}
\end{table}

\begin{table}[htb]
    \centering
    \begin{tabular}{|l|r|r|r|r|r|}\hline
    t=1 & 0.02 & 0.08 & 0.01 & 0.68 & 0.04 \\\hline
    t=2 & 0.05 & 0.06 & 0.69 & 0.02 & 0.01 \\\hline
    t=3 & 0.14 & 0.12 & 0.09 & 0.03 & 0.55 \\\hline
    t=4 & 0.16 & 0.09 & -0.00 & -0.00 & 0.01 \\\hline
    \end{tabular}
    \caption{GIv3: Qualitative comparison on Simple data}
    \label{tab:simple:giv3}
\end{table}

\subsection{Analysis of Simple setting with curvature}
Consider multiple features in the input and each feature `j' at the time step `t' agrees with the label `y' with the probability $p_j(t)$. 
The generative model setting is such that $log \frac{p_j(t)}{1-p_j(t)}$ has quadratic dependence with time and is given by $a_j^*t^2+b_j^*t+c_j^t$ for some latent values of $a_j^*, b_j^*, c_j^*$. By maximizing the data likelihood, we wish to estimate the values of `a, b, c'. We parametrize $p_j(t)$ as $\sigma(a_jt^2+b_jt+c_j)$  just as in the generative setting. Given the values of $a_j, b_j, c_j$, $p_j(t)$ is uniquely determined and also note that $p_j(t), p_j(t')$ are conditionally independent given the value of the coefficients. Log-Data likelihood takes the following form on the training data $\{X^t, Y^t\}_{t=1}^T$ for training steps ranging from 1 to T. 

\begin{align}
    \text{LL}(X, Y | a, b, c) &= \sum_{t=1}^{t=T} \sum_i \log\Pr(X^{ti}|Y^{ti}, a, b, c) + \log\Pr(Y^{ti})
\end{align}
Let $N_{j1}^t, N_{j0}^t$ be the number of times the $j^{th}$ feature agreed and disagreed with the label respectively at the $t^{th}$ step. We ignore the last term since the label prior does not depend on the parameters of our interest: a, b, c.
\begin{align}
    = \sum_t\sum_j N_{j1}^t\log(p_j(t)) + N_{j0}^t \log(1-p_j(t))\\
    p_j(t) = \sigma(a_jt^2+b_jt+c_j)
\end{align}
We estimate the values of `$a_j, b_j, c_j$' for each feature by maximizing the data likelihood shown above. 
Setting the derivative of LL with each of $a_j, b_j, c_j$, we obtain the following expressions, for some `j'. 

\begin{align}
    &\frac{\partial LL}{\partial a_j} = 0\nonumber\\
    &\implies \sum_t N_{j1}^t \frac{p_j(t)(1-p_j(t))}{p_j(t)}t^2 - N_{j0}\frac{p_j(t)(1-p_j(t))}{(1-p_j(t))}t^2=0\\
    &\text{Overall, doing the same for $b_j, c_j$, we get the following system of linear equations}\nonumber\\
    &\sum_t (N_{j1}^t - (N_{j1}^t + N_{j0}^t)p_j(t))t^2 = 0 \\
    &\sum_t (N_{j1}^t - (N_{j1}^t + N_{j0}^t)p_j(t))t = 0 \\
    &\sum_t (N_{j1}^t - (N_{j1}^t + N_{j0}^t)p_j(t))1 = 0
\end{align}
The vector $\vec{k} = [N_{j1}^1 - ( N_{j1}^1 + N_{j0}^1)p_j(1) \cdots, N_{j1}^T - (N_{j1}^T + N_{j0}^T)p_j(T)]^T$ should be in the null space of the matrix, denote Q, whose $t^{th}$ column is $[1, t, t^2]^T$, i.e. $Q\vec{k} = \mathbf{0}$. 

We will now consider a special case when T=3, the determinant of Q then is $(t_2-t_1)(t_3-t_1)(t_3-t_2)$ where $t_1, t_2, t_3$ are values determining the three train times. Since, no two times are the same Q is not singular, which means the solution to the above system of equations is the trivial 0 solution, i.e. $p_j(t)=\frac{N_{j1}^t}{N_{j1}^t+N_{j0}^t}$ for each `t'. Since $p_j(t)=\sigma(a_jt^2+b_jt+c_j)$. Since we have three (non-degenerate) observations, we can uniquely determine the values of $a_j, b_j, c_j$. 

It can be shown that in this setting, the Bayes optimal classifier takes the following form.
\begin{align}
f(x, t) &= \sum_j \log \frac{\Pr_j(t)}{1-\Pr_j(t)}x_j \nonumber\\
&= \sum_j (a_j^*t^2 + b_j^*t + c_j^*)x_j
\end{align}
The generalization performance depends on how close our estimated values are to the true values. For the Bayes optimal classifier, the generalization gap at time step `t'>T, is shown below. 

\begin{equation}
err(t) = \|\sum_j [(a_j^*-a_j)t^2 + (b_j^*-b_j)t + (c_j^*-c_j)] x_j\|
\end{equation}

The error value is qualified by estimation error on the coefficients. We will now try to express the error in the coefficients in a closed form. Denote $v_j^t$ such that $\sigma(v_j^t)=p_j(t)$, i.e. $v_j^t = \log\frac{p_j(t)}{1 - p_j(t)}$ obtained using the estimated value of $p_j(t) = \frac{N_{j1}^t}{N_{j1}^t+N_{j0}^t}$. We can obtain the value of coefficients by solving the following linear equations. Denote the three train time steps as $t_1, t_2, t_3$.

\begin{align}
\begin{bmatrix}
1 & t_1 & t_1^2 \\
1 & t_2 & t_2^2 \\
1 & t_3 & t_3^2 \\
\end{bmatrix}
\begin{bmatrix}
c_j \\
b_j \\
a_j
\end{bmatrix}
=\begin{bmatrix}
v_j^1 \\
v_j^2 \\
v_j^3
\end{bmatrix}\nonumber\\
\implies [a_j, b_j, c_j]^T = A\vec{v_j}\\
\text{with A appropriately defined}\nonumber
\end{align}

If we denote the $i^{th}$ row of A by $A_i$, the error on $a_j$ takes the following form.
\begin{align}
    err(a_j) &= A_1err(\vec{v_j})\nonumber\\
    err(\vec{v_j}) &= [\frac{(1-p_j(t))}{p_j(t)}\frac{1-p_j(t)+p_j(t)}{(1-p_j(t))^2}err(p_j(t))]_{t=1}^T \nonumber\\
    &= [\frac{err(p_j(t))}{p_j(t)(1-p_j(t))}]_{t=1}^T \nonumber\\
    err(p_j(t)) &= \frac{p_j^*(t)(1-p_j^*(t))}{N_{j0}^t + N_{j1}^t}\nonumber\\
    &\text{If we assume equal number of samples per time step, denoted N}\nonumber\\
    &\text{We assume $p_j(t)(1-p_j(t))\approx p_j^*(t)(1-p_j^*(t))$ }\nonumber\\
    \implies err(\vec{v_j}) &= [\frac{1}{N}]_{t=1}^T\nonumber\\
    \implies [err(a), err(b_j), err(c_j)]^T &= A\mathds{1}/N
    \label{eqn:err_t3}
\end{align}

In the case when there are three measurements and when fitting quadratic coefficient dynamics, we find that the estimation error is independent of the curvature, i.e. we do not see the effect of the value of `a' figuring in the generalization error. In other words, features with large curvature time dynamics need not necessarily lead to worse future time generalization. 

{\bf Discussion:}\\
In general, for T train time steps, we can fit $T-1^{th}$ degree polynomial with T parameters. The error in such a case takes the same form as was the case with T=3 shown in eqn.~\eqref{eqn:err_t3}. The estimation error on each of the polynomial coefficients is qualified by the average number of examples per time step: N. On the other extreme, consider the case when we fit a time independent term, i.e. $p_j(t)=\sigma(c_j)$. Following the same procedure as above of optimizing the likelihood value wrt $c_j$, we obtain the estimate of $c_j$ from the equation below. 

$$
\sigma(c_j) = \frac{\sum_t N_{j1}^t}{\sum_t N_{j1}^t + N_{j0}^t} = \frac{\sum_t N_{j1}^t}{TN}
$$

Consider also the case when the $j^{th}$ feature has almost constant correlation with time, i.e. $a_j*\approx 0, b_j^*\approx 0$. In such a case, the generalization error at t for the case of full parameterization: $err^{full}(t)$ and with only one constant parameterization: $err^{constant}(t)$ are contrasted below. 

\begin{align}
    err^{full}(t) &= err(a_j)t^2 + err(b_j)t + err(c_j)\nonumber\\
    err^{constant}(t) &= a_j^*t^2 + b_j^*t^2 + err(c_j)\nonumber
\end{align}
When $a_j^*\rightarrow 0, b_j^*\rightarrow 0$, the first two terms in $err^{full}$ will dominate first two in $err^{constant}$, note the $err(a_j), err(b_j)$ are independent of the value of $a_j, b_j$. Moreover, the error in $c_j$ for $err^{constant}$ is of the order $\mathcal{O}(1/TN)$ whereas is $\mathcal{O}(1/N)$ with full parameterization. As a result, the generalization error for any non-varying feature is far less with constant parameterization than with full. On the other hand, constant parameterization on any randomly picked feature could hurt if the feature varies a lot between the time steps, i.e. $a_j, b_j\not\approx 0$. In the same vein as constant parameterization, domain erasure methods learn time-invariant parameters and further encourage learning only the time-invariant features. Such a strong assumption on desirable features could compromise the classification performance.

The two extremes defined by the full and constant parameterization both have strong drawbacks and even better performance could be obtained by carefully controlling the fitting of time dynamics. 
{\it Intuition:} The $\delta_{max}$ of GI directly controls the capacity of the time-dependence of the feature since it controls the number of different lines used for fitting the dynamic. For example, when $\delta_{max}=T$, then we can only have weights constant or linear with time; when $\delta_{max}=0$, it is equivalent to full parameterization; when $\delta_{max}=T/2$, then the fit can only be pair of lines. Could GI be pitched as a method that enables trading off between fitting complex time-dependence of the feature and example sharing through reduced number of params, i.e. to navigate the region between constant and full parameterization.

\textbf{Dicussion 3/5/21:}

On the original toy setup, try other kind of regularization , e.g. suppressing the range of each feautre.
% As noted earlier, the analysis is for the case when T=3. The behaviour when T>3 is different and could be interesting. 
